A comparative study of uncertainty quantification methods in gust response analysis of a Lift-Plus-Cruise eVTOL aircraft wing

Wind gusts, being inherently stochastic, can significantly influence the safety and performance of aircraft. This study investigates a three-dimensional uncertainty quantification (UQ) problem to explore how uncertainties in gust and flight conditions affect the structural response of a Lift-Plus-Cruise eVTOL aircraft wing. The analysis employs an unsteady aeroelastic model with a one-way coupling between a panel method aerodynamic solver and a shell analysis structural solver to predict the wing's response under varying conditions. Additionally, this paper presents a comparative evaluation of commonly used non-intrusive UQ methods, including non-intrusive polynomial chaos, kriging, Monte Carlo, univariate dimension reduction, and gradient-enhanced univariate dimension reduction. These methods are assessed based on their effectiveness in estimating various risk measures-mean, standard deviation, and 95th percentile-of critical structural response outputs such as maximum tip displacement and average strain energy. The numerical results reveal significant variability in the structural response outputs, even under relatively small ranges of uncertain inputs. This highlights the sensitivity of the system to uncertainties in gust and flight conditions. Furthermore, the performance of the implemented UQ methods varies significantly depending on the specific risk measures and the quantity of interest being analyzed.

==> sections/outline.tex <==
\section{Outline}
\begin{itemize}
    \item Goal: perform a comparative study on common non-adaptive UQ methods for two aerodynamic analysis problem
    \item First problem: steady aerodynamic UQ analysis problem with VLM (3D)
    \item Third problem: Gust response UQ analysis with UVLM (4D)
    \item Compared method: NIPC (integration-based + regression-based), kriging, Monte Carlo, First-order approximation, UDR, GUDR 
\end{itemize}

\section{Problem descriptions}
% \subsection{UQ problem 1, steady aerodynamic UQ analysis problem with VLM}
% \textbf{Objective:} The objective of this problem is to perform an uncertainty quantification (UQ) analysis on the steady-state aerodynamic performance of an aircraft, given uncertainties in the Mach number, altitude, and angle of attack. The primary quantities of interest (QoIs) are the lift coefficient (\(C_L\)) and drag coefficient (\(C_D\)).

% \subsection{Problem Overview:}
% In steady-state aerodynamic performance, the lift and drag coefficients are critical for understanding the overall aerodynamic efficiency of an aircraft. These coefficients depend on various design and environmental parameters, such as the Mach number, altitude, and angle of attack. We seek to estimate the mean, standard deviation, and 99th percentile of \(C_L\) and \(C_D\) under uncertainty in the input variables.
\subsection{Problem 1: 3D UQ aerodynamics analysis problem with steady VLM}
In this problem, we focus on a steady-state aerodynamic analysis of a wing using the Vortex Lattice Method (VLM). The goal is to quantify the uncertainty in the lift coefficient (\(C_L\)) and drag coefficient (\(C_D\)) due to uncertainties in the input parameters.
\begin{itemize}
    \item Model: steady VLM
    \item Uncertain inputs: mach Number (\(M\)), altitude (\(h\)), angle of attack (\(\alpha\))
    \item QoIs: \(C_L\),  \(C_D\)
    \item Risk measures: mean, standard deviation, 99 percentile
\end{itemize}

\subsection{Problem 2: 4D UQ gust response analysis problem with unsteady VLM}
This problem focuses on the unsteady aerodynamic analysis of a wing subjected to gust wind disturbances. The Unsteady Vortex Lattice Method (UVLM) is used to simulate the aerodynamic response of the wing under gust conditions. The objective is to quantify the uncertainty in the maximum lift coefficient (\(C_L\)) and the total energy of the lift coefficient over time due to uncertainties in the gust characteristics and flight conditions.
\begin{itemize}
    \item Model: unsteady VLM
    \item Uncertain inputs: gust amplitude (\(A\)), gust frequency (\(f\)), mach number (\(M\)), altitude (\(h\))
    \item QoIs: Maximum lift coefficient (\(C_L^{\text{max}}\)), total energy of the lift coefficient (\(E_{C_L}\))
    \item Risk measures: mean, standard deviation, 99 percentile
\end{itemize}

\section{Ideas}
\begin{itemize}
    \item To increase UQ dimensions: geometry uncertainties?
    \item To make a problem that favours AMTC? Fuel consumption estimation for a cruise mission?
\end{itemize}
